Microstructurally-based constitutive modelling of the skin - Linking intrinsic ageing to microstructural parameters

A multiphasic constitutive model of the skin that implicitly accounts for the process of intrinsic (i.e.\ chronological) ageing via variation of the constitutive parameters is proposed. The structurally-motivated constitutive formulation features distinct mechanical contributions from collagen and elastin fibres. The central hypothesis underpinning this study is that the effects of ageing on the mechanical properties of the tissue are directly linked to alterations in the microstructural characteristics of the collagen and elastin networks. Constitutive parameters in the model, corresponding to different ages, are identified from published experimental data on bulge tests of human skin. The identification procedure is based on an inverse finite element method. The numerical results demonstrate that degradation of the elastin meshwork and variations in anisotropy of the collagen network are plausible mechanisms to explain ageing in terms of macroscopic tissue stiffening. Whereas alterations in elastin affect the low-modulus region of the skin stress-strain curve, those related to collagen have an impact on the linear region.

==> packages_style_defs.tex <==
%\usepackage{graphicx,psfrag,epsfig,rotating}
\usepackage{color}

%\usepackage{booktabs}
%\usepackage{url}
%\usepackage{longtable}

%\usepackage[latin1]{inputenc}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{nomencl}
\usepackage{lscape}
%\usepackage{soul}
\usepackage{tabularx}
\usepackage{pdflscape}
\usepackage{upgreek}

%\usepackage{array,float,latexsym,amsmath,amssymb,amsbsy,eurosym,theorem,amsfonts,mathrsfs,bbm,verbatim}

%\usepackage{SIunits}

%\usepackage{ngerman,oldgerm,german}

\usepackage[active]{srcltx}

\usepackage{pdfsync}

%\usepackage{arcs}
%\usepackage{phonetic}

%\pagestyle{plain}
%\usepackage{lineno}

\DeclareMathOperator{\sgn}{sgn}

\newcommand{\dfracp}[2]{\dfrac{\partial #1}{\partial#2}}
\newcommand{\jmp}[1]{[\![ {#1} ]\!]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\eqn}[1]{Eq.~(\ref{#1})}
\newcommand{\eqns}[1]{Eq.~(\ref{#1})}
\newcommand{\eqnsab}[2]{Eq.~(\ref{#1})--(\ref{#2})}
\newcommand{\subeqn}[2]{Eq.~(\ref{#1})${}_#2$}
\newcommand{\fig}[1]{Fig.~\ref{#1}}
\newcommand{\figs}[1]{Fig.~\ref{#1}}
\newcommand{\sect}[1]{Sec.~\ref{#1}}
\newcommand{\sects}[2]{Sec.~\ref{#1} and \ref{#2}}
\newcommand{\tableref}[1]{Table~\ref{#1}}
\newcommand{\chp}[1]{Chapter~\ref{#1}}
\newcommand{\chps}[2]{Chapters~\ref{#1} and \ref{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      BOLD OPERATORS    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\renewcommand{\b}[1]{\mathbf{#1}} % mathbf doesn't work on greek letters! it is bold but not italic.
\renewcommand{\b}[1]{\boldsymbol{#1}} % it is bold and italic on latin letters. also, works on greek letters.


%\renewcommand{\c}[1]{\mathcal{#1}}
\newcommand{\s}[1]{\mathscr{#1}}
\newcommand{\B}[1]{\boldsymbol{\mathcal{#1}}}
\renewcommand{\v}[1]{\mathbbm{#1}} % blackboard (double-barred) font

\newcommand{\h}[1]{\widehat{#1}}
\renewcommand{\u}[1]{\underline{#1}}
\renewcommand{\t}[1]{\widetilde{#1}}
\renewcommand{\u}[1]{\underline{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      BOLD GREEK & LATIN LETTERS    %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lrp}[1]{\left( {#1} \right)}
\newcommand{\lb}{\left[}
\newcommand{\rb}{\right]}
\newcommand{\lrb}[1]{\left[ {#1} \right]}
\newcommand{\lrrb}[1]{\left( {#1} \right)}
\newcommand{\lrvb}[1]{\left| {#1} \right|}
\newcommand{\lc}{\left\{}
\newcommand{\rc}{\right\}}
\newcommand{\lrc}[1]{\left\{ {#1} \right\}}

\newcommand{\p}{\partial}

\newcommand{\f}{\displaystyle\frac}
\newcommand{\tf}{\tfrac}
\newcommand{\df}{\dfrac}
%\newcommand{\dfracp}[2]{ {\partial_{#2}{#1}}}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
\newcommand{\infrac}[2]{{#1}/{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bnull}{\b0}

\newcommand{\de}{\delta}

\newcommand{\Dt}{\mbox{D}_t}
\newcommand{\dt}{\mbox{d}_t}
\renewcommand{\d}{\mathsf{d}}
%\newcommand{\D}{\mbox{D}}
%\newcommand{\grad}{\ensuremath{\mbox{grad}}}
\newcommand{\grad}{\nabla}
\newcommand{\gradsym}{\nabla_{\vx}^{\mbox{\scriptsize sym}}}
\renewcommand{\div}{\mbox{div}}
\newcommand{\curl}{\mbox{curl}}
\newcommand{\Grad}{\ensuremath{\mbox{Grad}}}
%\newcommand{\Grad}{\nabla_{\vX}}
\newcommand{\Gradsym}{\Grad^{\mbox{\scriptsize sym}}}
\newcommand{\Div}{\mbox{Div}}
\newcommand{\Lin}{\mbox{Lin}}
\newcommand{\Tr}{\mbox{Tr}}
\newcommand{\tr}{\mbox{tr}}

\newcommand{\dyad}{\otimes}

\newcommand{\xt}{{}^{{\!\!\mbox{\scriptsize ext}}}}
\newcommand{\nt}{{}^{{\!\!\mbox{\scriptsize int}}}}
\newcommand{\sym}{{\mbox{\scriptsize sym}}}
\newcommand{\vol}{{\mbox{\scriptsize vol}}}
\newcommand{\dev}{{\mbox{\scriptsize dev}}}
\newcommand{\eff}{{\mbox{\scriptsize eff}}}

\newcommand{\prs}{{}^{\mbox{\scriptsize p}}} % prescribed
\newcommand{\happ}{{}^{h}} % h for approximation
\newcommand{\nnn}{{}^{\text{\scriptsize nn}}} % h for approximation

\newcommand{\inv}{{}^{-\text{\scriptsize 1}}}
\newcommand{\trns}{{}^{\mathsf{\scriptsize T}}}
\newcommand{\Trns}{{}^{\text{\scriptsize T}}}
\newcommand{\invtrns}{{}^{-\text{\scriptsize T}}}

\newcommand{\Det}{\text{Det}}
\newcommand{\Cof}{\text{Cof}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Ae}{\mathop{\mbox{\LARGE {\textsf {\textbf A}}}}_{e} }
\newcommand{\bulkassembly}{\mathop{\mbox{\LARGE {\textsf {\textbf A}}}}_{\beta=1}^{n_{\mbox{\scriptsize b.el}}} }
\newcommand{\interfaceassembly}{\mathop{\mbox{\LARGE {\textsf {\textbf A}}}}_{\gamma=1}^{n_{\mbox{\scriptsize i.el}}} }
\newcommand{\surfaceassembly}{\mathop{\mbox{\LARGE {\textsf {\textbf A}}}}_{\gamma=1}^{n_{\mbox{\scriptsize s.el}}} }

\newcommand{\bdsp}{{\mbox{{\textsf {\textbf d}}}}}

\newcommand{\bres}{{\mbox{{\textsf {\textbf R}}}}}
\newcommand{\res}{{\mbox{{\textsf { R}}}}}

\newcommand{\ovres}{\, \intr{\mbox{{\textsf {\textbf R}}}}}
\newcommand{\ores}{\, \intr{\mbox{{\textsf {R}}}}}

\newcommand{\bstf}{{\mbox{{\textsf {\textbf K}}}}}
\newcommand{\stf}{{\mbox{{\textsf { K}}}}}

\newcommand{\hsth}{\{\h\bullet\}}
\newcommand{\osth}{\{\o\bullet\}}
\newcommand{\tsth}{\{\t\bullet\}}
\newcommand{\sth}{\{\bullet\}}

\newcommand{\hstH}{\{\h\circ\}}
\newcommand{\ostH}{\{\o\circ\}}
\newcommand{\tstH}{\{\t\circ\}}
\newcommand{\stH}{\{\circ\}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      COLORS    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\hide #1{{\color[rgb]{1,1,1} #1}}

\definecolor{gray}{rgb}{0.75, 0.75, 0.75}
\definecolor{yellow}{rgb}{1, 0.7, 0.2}
\definecolor{green}{rgb}{0.3, 0.9, 0.3}
\definecolor{brown}{rgb}{0.6, 0.3, 0.2}
\definecolor{magenta}{rgb}{0.9, 0.1, 0.9}
\definecolor{light}{rgb}{1, 0.7, 0.7}

\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%      BOXES AND EQUATIONS    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% boxed equation white color
\newcommand{\beqwc}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}

% boxed equation* white color
\newcommand{\beqqwc}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-2\fboxsep}%
      \addtolength{\linewidth}{-2\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation*}#1\end{equation*}%
      \end{minipage}%
    }\]%
}

% boxed equation (default) with gray inside
\newcommand{\beq}[1]{%
  \[\fbox{%
      \addtolength{\linewidth}{-1\fboxsep}%
      \addtolength{\linewidth}{-1\fboxrule}%
      \begin{minipage}{\linewidth}%
      \begin{equation}#1\end{equation}%
      \end{minipage}%
    }\]%
}

